Trajectory Optimization and Following for a Three Degrees of Freedom Overactuated Floating Platform

Space robotics applications, such as Active Space Debris Removal (ASDR), require representative testing before launch. A commonly used approach to emulate the microgravity environment in space is air-bearing based platforms on flat-floors, such as the European Space Agency's Orbital Robotics and GNC Lab (ORGL). This work proposes a control architecture for a floating platform at the ORGL, equipped with eight solenoid-valve-based thrusters and one reaction wheel. The control architecture consists of two main components: a trajectory planner that finds optimal trajectories connecting two states and a trajectory follower that follows any physically feasible trajectory. The controller is first evaluated within an introduced simulation, achieving a 100 % success rate at finding and following trajectories to the origin within a Monte-Carlo test. Individual trajectories are also successfully followed by the physical system. In this work, we showcase the ability of the controller to reject disturbances and follow a straight-line trajectory within tens of centimeters.

==> content/weight_matrices.tex <==
%!TEX root = ../root.tex
\subsection*{Weight Matrices}\label{appendix:weightmatrices}

\begin{table}[ht]
	\centering
	\resizebox{0.5\textwidth}{!}{
	\begin{tabular}{@{}ll@{}}\hline
	& Simulation \\\hline\hline
	$Q_{kf}$ & Diag$\left(\begin{bmatrix}
	                0.1 & 0.1 & & 0.1 & 0.1 & 0.1 & 0.1 & 1
	             \end{bmatrix}\right)$\\
	$R_{kf}$ & Diag$\left(\begin{bmatrix}
	                \num{1e-3} & \num{1e-3} & \num{1e-3} & \num{5e3} & \num{5e3} & \num{5e3} & 1
				  \end{bmatrix}\right)$\\
	$Q_{TVLQR}$ & Diag$\left(\begin{bmatrix}
	                \num{1e4} & \num{1e4} & \num{1e4} & 100 & 100 & 100 & \num{1e-3}
				  \end{bmatrix}\right)$\\
	$Q_{final}$ & Diag$\left(\begin{bmatrix}
	                \num{1e5} & \num{1e5} & \num{1e5} & \num{1e6} & \num{1e6} & \num{1e6} & \num{1e-7}
				  \end{bmatrix}\right)$\\
	$R_{TVLQR}$ & Diag$\left(\begin{bmatrix}
	                \num{1e1} & \num{1e1} & \num{1e1} & \num{1e1} & \num{1e1} & \num{1e1} & \num{1e1} & \num{1e1} & \num{1e1}\\
				  \end{bmatrix}\right)$\\
	$R_{final}$ & Diag$\left(\begin{bmatrix}
	                \num{1} & \num{1} & \num{1} & \num{1} & \num{1} & \num{1} & \num{1} & \num{1} & \num{1}\\
				  \end{bmatrix}\right)$\\\hline
	 & Real System \\\hline\hline
	 $Q_{kf}$ & Diag$\left(\begin{bmatrix}
	                0.1 & 0.1 & & 0.1 & 0.1 & 0.1 & 0.1 & 1
	             \end{bmatrix}\right)$\\
	$R_{kf}$ & Diag$\left(\begin{bmatrix}
	                \num{1e-3} & \num{1e-3} & \num{1e-3} & \num{5e3} & \num{5e3} & \num{5e3} & 1
				  \end{bmatrix}\right)$\\
	$Q_{TVLQR}$ & Diag$\left(\begin{bmatrix}
	                \num{5e3} & \num{5e3} & \num{5e2} & \num{5e2} & \num{5e2} & \num{2e3} & \num{1e-3}
				  \end{bmatrix}\right)$  \\
	$Q_{final}$ & Diag$\left(\begin{bmatrix}
	                \num{5e3} & \num{5e3} & \num{5e2} & \num{5e2} & \num{5e2} & \num{2e3} & \num{1e-3}
				  \end{bmatrix}\right)$  \\
	$R_{TVLQR}$ & Diag$\left(\begin{bmatrix}
	                \num{1} & \num{200} & \num{200} & \num{200} & \num{200} & \num{200} & \num{200} & \num{200} & \num{200}\\
				  \end{bmatrix}\right)$\\
	$R_{final}$ & Diag$\left(\begin{bmatrix}
	                \num{1} & \num{200} & \num{200} & \num{200} & \num{200} & \num{200} & \num{200} & \num{200} & \num{200}\\
				  \end{bmatrix}\right)$\\\hline
	\end{tabular}
	}
	\caption{Weight Matrices used for the observer and controller for the simulation and the real-system}
	\label{tab:weight-Matrices}
\end{table}

